IBIA: Bayesian Inference via Incremental Build-Infer-Approximate operations on Clique Trees

Exact inference in Bayesian networks is intractable and has an exponential dependence on the size of the largest clique in the corresponding clique tree (CT), necessitating approximations. Factor based methods to bound clique sizes are more accurate than structure based methods, but expensive since they involve inference of beliefs in a large number of candidate structure or region graphs. We propose an alternative approach for approximate inference based on an incremental build-infer-approximate (IBIA) paradigm, which converts the Bayesian network into a data structure containing a sequence of linked clique tree forests (SLCTF), with clique sizes bounded by a user-specified value. In the incremental build stage of this approach, CTFs are constructed incrementally by adding variables to the CTFs as long as clique sizes are within the specified bound. Once the clique size constraint is reached, the CTs in the CTF are calibrated in the infer stage of IBIA. The resulting clique beliefs are used in the approximate phase to get an approximate CTF with reduced clique sizes. The approximate CTF forms the starting point for the next CTF in the sequence. These steps are repeated until all variables are added to a CTF in the sequence. We prove that our algorithm for incremental construction of clique trees always generates a valid CT and our approximation technique preserves the joint beliefs of the variables within a clique. Based on this, we show that the SLCTF data structure can be used for efficient approximate inference of partition function and prior and posterior marginals. More than 500 benchmarks were used to test the method and the results show a significant reduction in error when compared to other approximate methods, with competitive runtimes.

==> tables/avg.tex <==
\begin{table}[!htp]\centering
    \caption{Average statistics obtained with different approximate inference methods for various benchmarks.\textcolor{red}{Fix zeros}}\label{tab:avgStats}
\scriptsize
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|r|rrrrrrrr|}\toprule
    \bf Query & \bf Benchmark   &\textbf{Method} &\textbf{\#Inst.} &\textbf{Avg.$\boldsymbol{\Delta_{PR}}$} &\textbf{Avg. MaxErr} &\textbf{Avg. RMSE} &\textbf{Avg. KLmean} &\textbf{Avg. KLmax} &\textbf{Avg. Runtime} \\\midrule
    \multirow{18}{*}{\textbf{MAR\_e}} &\multirow{6}{*}{\textbf{BN\_UAI}}& FBP &90 &0.27 &0.207 &0.039 &0.035 &3.080 &33 \\
& &WMB &90 &2.55 &0.202 &0.046 &0.004 &0.141 &239 \\
& &IJGP &81 &- &0.326 &0.079 &0.245 &5.050 &148 \\
& &Gibbs &90 &- &0.420 &0.146 &0.048 &3.630 &6 \\
& &WMB10 &90 &5.53 &0.288 &0.078 &0.008 &0.209 &8 \\
  \rowcolor{gray!40}   & &IBIA &90 &2.53$\times 10^{\mbox{-4}}$ &0.006 &6.67$\times 10^{\mbox{-4}}$ &4.67$\times 10^{\mbox{-6}}$ &0.003 &4 \\ \cmidrule{2-10}
&\multirow{6}{*}{\textbf{Pedigree}} &FBP &9 &2.25 &0.520 &0.189 &0.623 &41.200 &15 \\
& &WMB &5 &0.93 &0.174 &0.018 &4.86$\times 10^{\mbox{-4}}$ &0.099 &836 \\
& &IJGP &5 &- &0.490 &0.135 &0.267 &7.570 &411 \\
& &Gibbs &9 &- &0.998 &0.436 &1.880 &15.900 &7 \\
& &WMB10 &9 &5.22 &0.421 &0.064 &0.004 &0.303 &26 \\ 
 \rowcolor{gray!40}    & &IBIA &9 &0.12 &0.237 &0.028 &6.67$\times 10^{\mbox{-4}}$ &0.151 &18 \\  \cmidrule{2-10}
&\multirow{6}{*}{\textbf{Relational}} &FBP &392 &1 &0.449 &0.123 &0.295 &11.101 &51 \\
& &WMB &227 &4 &0.112 &0.019 &0.001 &0.072 &481 \\
& &IJGP &203 &- &0.287 &0.082 &0.306 &4.319 &376 \\
& &Gibbs &395 &- &0.811 &0.337 &0.098 &1.176 &243 \\
& &WMB10 &272 &19 &0.330 &0.088 &0.017 &0.632 &216 \\
 \rowcolor{gray!40}    & &IBIA &384 &0.1 &0.146 &0.036 &0.010 &0.781 &147 \\ \midrule
\multirow{24}{*}{\textbf{MAR\_p}} &\multirow{6}{*}{\textbf{BN\_UAI}} &FBP &76 &- &0.169 &0.036 &0.003 &0.114 &151 \\
& &WMB &76 &- &0.254 &0.073 &0.007 &0.188 &449 \\
& &IJGP &65 &- &0.527 &0.165 &0.767 &8.210 &235 \\
& &Gibbs &76 &- &0.454 &0.142 &0.036 &3.660 &9 \\
& &WMB10 &76 &- &0.312 &0.104 &0.012 &0.251 &30 \\
 \rowcolor{gray!40}    & &IBIA &76 &- &0.015 &0.001 &5.08$\times 10^{\mbox{-6}}$ &0.007 &4 \\  \cmidrule{2-10}
&\multirow{6}{*}{\textbf{GridBN}} &FBP &29 &- &0.474 &0.109 &0.010 &0.400 &0 \\
& &WMB &29 &- &0.427 &0.095 &0.007 &0.288 &373 \\
& &IJGP &24 &- &0.746 &0.235 &0.893 &11.800 &256 \\
& &Gibbs &29 &- &0.919 &0.388 &1.400 &13.300 &6 \\
& &WMB10 &29 &- &0.520 &0.146 &0.015 &0.355 &4 \\
  \rowcolor{gray!40}   & &IBIA &29 &- &8.62$\times 10^{\mbox{-4}}$ &3.45$\times 10^{\mbox{-5}}$ &2.09$\times 10^{\mbox{-8}}$ &3.84$\times 10^{\mbox{-4}}$ &2 \\  \cmidrule{2-10}
&\multirow{6}{*}{\textbf{Bnlearn}} &FBP &26 &- &0.068 &0.010 &3.13$\times 10^{\mbox{-4}}$ &0.037 &0 \\
& &WMB &26 &- &0 &0 &8.48$\times 10^{\mbox{-9}}$ &6.73$\times 10^{\mbox{-7}}$ &9 \\
& &IJGP &26 &- &0 &0 &6.79$\times 10^{\mbox{-9}}$ &6.81$\times 10^{\mbox{-7}}$ &7 \\
& &Gibbs &26 &- &0.511 &0.171 &0.257 &6.610 &2 \\
& &WMB10 &26 &- &0.028 &0.005 &2.59$\times 10^{\mbox{-4}}$ &0.016 &22 \\
    \rowcolor{gray!40}& &IBIA &26 &- &0.003 &2.69$\times 10^{\mbox{-4}}$ &2.06$\times 10^{\mbox{-6}}$ &0.001 &0 \\ \cmidrule{2-10}
    &  \multirow{6}{*}{\textbf{Relational}} &FBP &386 &- &0.592 &0.205 &0.208 &7.054 &15 \\
& &WMB &194 &- &0.199 &0.05 &0.003 &0.135 &497 \\
& &IJGP &168 &- &0.648 &0.222 &0.958 &9.619 &315 \\
& &Gibbs &386 &- &0.758 &0.297 &0.058 &0.873 &241 \\
& &WMB10 &242 &- &0.529 &0.171 &0.035 &1.135 &222 \\
 \rowcolor{gray!40}& &IBIA &386 &- &0.314 &0.087 &0.027 &2.013 &127 \\ 
\bottomrule
\end{tabular}%
    }
\end{table}


==> tables/cmpCliqueSize.tex <==
% !TeX spellcheck = en_US
\begin{table}[!htp]\centering
\caption{Comparison of maximum error, RMSE and required runtime for inference of prior marginals using various clique size constraints. Number of partitions in each case is indicated in  brackets. We report errors upto three decimal places. The error is reported as 0 when it is $<10^{-16}$. Entries are marked with dash if the maximum factor size of CPTs $>mcs_p$.}\label{tab:mcsthComparison}
\scriptsize
\setlength\tabcolsep{2pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|cc>{\columncolor{gray!30}}cc|cc>{\columncolor{gray!30}}cc|cc>{\columncolor{gray!30}}cc|}\toprule
	\textbf{} &\multicolumn{4}{c|}{\textbf{Maximum Error (\#Partitions)}} &\multicolumn{4}{c|}{\textbf{RMSE}} &\multicolumn{4}{c|}{\textbf{Runtime}} \\\cmidrule{2-13}
	$\mathbf{(mcs_p, mcs_{im})}$ &\textbf{(10,5)} &\textbf{(15,10)} &\textbf{(20,15)} &\textbf{(25,20)} &\textbf{(10,5)} &\textbf{(15,10)} &\textbf{(20,15)} &\textbf{(25,20)} &\textbf{(10,5)} &\textbf{(15,10)} &\textbf{(20,15)} &\textbf{(25,20)} \\\midrule
BN\_55 &0.086 (8) &0.086 (9) &0.026 (7) &0.008 (8) &0.01 &0.007 &0.002 &0.001 &0.9 &1.2 &2.8 &59.9 \\
BN\_62 &0.094 (7) &0.05 (4) &0.056 (3) &0.038 (3) &0.012 &0.007 &0.004 &0.002 &1.7 &1.6 &3.2 &24.6 \\
BN\_51 &0.076 (5) &0.058 (4) &0.034 (3) &<0.001 (2) &0.013 &0.007 &0.003 &<0.001 &1.8 &1.6 &3.1 &49.0 \\
BN\_21 &- &0.067 (170) &0.06 (3) &0 (1) &- &0.003 &0.001 &0 &- &20.7 &10.3 &10.0 \\
mastermind\_03\_08\_03-0010 &0.067 (3) &0.059 (3) &0.044 (2) &0 (1) &0.019 &0.016 &0.005 &0 &5.9 &3.2 &2.6 &4.3 \\
mastermind\_03\_08\_04-0010 &0.09 (7) &0.087 (5) &0.088 (4) &0.057 (3) &0.022 &0.021 &0.02 &0.012 &18.7 &4.2 &6.5 &62.0 \\
mastermind\_03\_08\_05-0010 &0.093 (7) &0.104 (8) &0.13 (6) &0.118 (5) &0.021 &0.021 &0.028 &0.024 &6.5 &57.2 &11.2 &128.9 \\
blockmap\_15\_01-0006 &0.602 (20) &0.485 (13) &0.189 (8) &0.113 (9) &0.193 &0.111 &0.03 &0.018 &32.8 &41.4 &77.0 &796.0 \\
blockmap\_10\_01-0005 &0.364 (15) &0.361 (7) &0.222 (7) &<0.001 (5) &0.12 &0.075 &0.02 &<0.001 &8.6 &11.5 &23.2 &205.2 \\
90-23-5 &0.011 (7) &<0.001 (5) &0.002 (4) &<0.001 (4) &0.001 &<0.001 &<0.001 &<0.001 &0.5 &0.6 &1.2 &11.2 \\
90-42-5 &0.021 (11) &0.001 (11) &0.003 (10) &<0.001 (11) &0.002 &<0.001 &<0.001 &<0.001 &1.9 &2.4 &4.6 &67.5 \\
munin1 &0.142 (4) &0.104 (5) &0.017 (4) &0.001 (2) &0.009 &0.006 &0.002 &<0.001 &0.2 &0.2 &0.2 &1.0 \\
diabetes &- &0.043 (24) &0.049 (23) &0.001 (11) &- &0.01 &0.005 &<0.001 &- &0.7 &1.1 &4.5 \\
munin4 &0.088 (4) &0.054 (3) &<0.001 (2) &0 (1) &0.004 &0.002 &<0.001 &0 &0.7 &0.7 &0.8 &0.8 \\
	\bottomrule
\end{tabular}%
}
\end{table}

==> tables/cmpCliqueSizeAll.tex <==
% !TeX spellcheck = en_US
\begin{table}[!htp]\centering
\caption{Comparison of maximum error, RMSE and required runtime for inference of prior marginals using various clique size constraints. Number of partitions in each case is indicated in  brackets. We report errors upto three decimal places. The error is reported as 0 when it is $<10^{\mbox{-}16}$. Entries are marked with dash if the maximum factor size of CPTs $>mcs_p$.}\label{tab:mcsthComparisonAll}
\scriptsize
\setlength\tabcolsep{2pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|cc>{\columncolor{gray!30}}cc|cc>{\columncolor{gray!30}}cc|cc>{\columncolor{gray!30}}cc|}\toprule
	\textbf{} &\multicolumn{4}{c|}{\textbf{Maximum Error (\#Partitions)}} &\multicolumn{4}{c|}{\textbf{RMSE}} &\multicolumn{4}{c|}{\textbf{Runtime}} \\\cmidrule{2-13}
	$\mathbf{(mcs_p, mcs_{im})}$ &\textbf{(10,5)} &\textbf{(15,10)} &\textbf{(20,15)} &\textbf{(25,20)} &\textbf{(10,5)} &\textbf{(15,10)} &\textbf{(20,15)} &\textbf{(25,20)} &\textbf{(10,5)} &\textbf{(15,10)} &\textbf{(20,15)} &\textbf{(25,20)} \\\midrule
BN\_91 &- (-) &- (-) &$3\times 10^{\mbox{-}12}$ (4) &$1\times 10^{\mbox{-}13}$ (1) &- &- &$2\times 10^{\mbox{-}13}$ &$8\times 10^{\mbox{-}15}$ &- &- &2 &11 \\
BN\_93 &- (-) &- (-) &$3\times 10^{\mbox{-}11}$ (2) &$8\times 10^{\mbox{-}14}$ (1) &- &- &$1\times 10^{\mbox{-}12}$ &$9\times 10^{\mbox{-}15}$ &- &- &3 &7 \\
BN\_125 &- (-) &- (-) &0.001 (10) &$2\times 10^{\mbox{-}14}$ (1) &- &- &$3\times 10^{\mbox{-}4}$ &$4\times 10^{\mbox{-}15}$ &- &- &5 &18 \\
BN\_33 &0.160 (10) &0.002 (12) &$5\times 10^{\mbox{-}5}$ (11) &$2\times 10^{\mbox{-}7}$ (9) &0.009 &$7\times 10^{\mbox{-}5}$ &$2\times 10^{\mbox{-}6}$ &$2\times 10^{\mbox{-}8}$ &2 &2 &4 &55 \\
BN\_37 &0.061 (11) &0.131 (11) &0.002 (10) &$5\times 10^{\mbox{-}6}$ (8) &0.005 &0.005 &$2\times 10^{\mbox{-}4}$ &$1\times 10^{\mbox{-}7}$ &2 &2 &5 &66 \\
BN\_40 &0.049 (10) &0.009 (11) &0.001 (10) &$3\times 10^{\mbox{-}7}$ (9) &0.005 &$5\times 10^{\mbox{-}4}$ &$4\times 10^{\mbox{-}5}$ &$2\times 10^{\mbox{-}8}$ &2 &2 &5 &71 \\
BN\_43 &0.028 (6) &0.017 (5) &0.004 (4) &$1\times 10^{\mbox{-}4}$ (2) &0.004 &0.002 &$2\times 10^{\mbox{-}4}$ &$8\times 10^{\mbox{-}6}$ &1 &1 &2 &16 \\
BN\_51 &0.077 (5) &0.058 (4) &0.035 (3) &$1\times 10^{\mbox{-}16}$ (2) &0.013 &0.007 &0.003 &$9\times 10^{\mbox{-}18}$ &2 &2 &3 &49 \\
BN\_55 &0.086 (8) &0.086 (9) &0.026 (7) &$8\times 10^{\mbox{-}3}$ (8) &0.01 &0.007 &0.002 &$7\times 10^{\mbox{-}4}$ &1 &1 &3 &60 \\
BN\_62 &0.094 (7) &0.050 (4) &0.056 (3) &0.038 (3) &0.013 &0.007 &0.004 &0.002 &2 &2 &3 &25 \\
BN\_64 &0.115 (7) &0.064 (8) &0.011 (8) &0.005 (8) &0.013 &0.007 &$9\times 10^{\mbox{-}4}$ &$6\times 10^{\mbox{-}4}$ &1 &1 &3 &65 \\
BN\_66 &0.124 (8) &0.124 (10) &0.113 (10) &0.009 (9) &0.008 &0.007 &0.007 &$6\times 10^{\mbox{-}4}$ &1 &1 &4 &70 \\
mastermind\_10\_08\_03-0010 &0.042 (10) &0.015 (7) &0.011 (7) &0.008 (9) &0.004 &0.003 &0.002 &0.001 &20 &46 &24 &463 \\
mastermind\_10\_08\_03-0002 &0.030 (8) &0.014 (11) &0.017 (7) &0.009 (10) &0.003 &0.002 &0.002 &0.002 &43 &47 &23 &457 \\
mastermind\_05\_08\_03-0009 &0.040 (4) &0.033 (4) &0.021 (2) &0.021 (3) &0.009 &0.009 &0.005 &0.003 &13 &18 &9 &64 \\
mastermind\_06\_08\_03-0010 &0.041 (7) &0.026 (4) &0.021 (4) &0.015 (3) &0.007 &0.004 &0.005 &0.003 &8 &7 &32 &162 \\
mastermind\_04\_08\_03-0010 &0.052 (4) &0.030 (3) &0.036 (3) &0.004 (2) &0.013 &0.007 &0.008 &$3\times 10^{\mbox{-}4}$ &11 &10 &7 &29 \\
mastermind\_03\_08\_03-0010 &0.067 (3) &0.059 (3) &0.044 (2) &$3\times 10^{\mbox{-}15}$ (1) &0.019 &0.016 &0.005 &$2\times 10^{\mbox{-}16}$ &6 &3 &3 &4 \\
blockmap\_05\_03-0003 &0.603 (9) &0.142 (5) &$1\times 10^{\mbox{-}15}$ (5) &$1\times 10^{\mbox{-}15}$ (3) &0.168 &0.026 &$1\times 10^{\mbox{-}16}$ &$1\times 10^{\mbox{-}16}$ &1 &1 &2 &1 \\
blockmap\_15\_01-0006 &0.602 (20) &0.485 (13) &0.189 (8) &0.113 (9) &0.193 &0.111 &0.03 &0.018 &33 &41 &77 &794 \\
blockmap\_10\_01-0005 &0.364 (15) &0.361 (7) &0.222 (7) &$3\times 10^{\mbox{-}16}$ (5) &0.12 &0.075 &0.02 &$8\times 10^{\mbox{-}17}$ &8 &12 &23 &205 \\
90-42-5 &0.021 (11) &0.001 (11) &0.003 (10) &$6\times 10^{\mbox{-}7}$ (11) &0.002 &$1\times 10^{\mbox{-}4}$ &$1\times 10^{\mbox{-}4}$ &$3\times 10^{\mbox{-}8}$ &2 &2 &5 &67 \\
90-23-5 &0.011 (7) &$4\times 10^{\mbox{-}8}$ (5) &0.002 (4) &$5\times 10^{\mbox{-}8}$ (4) &0.001 &$6\times 10^{\mbox{-}9}$ &$2\times 10^{\mbox{-}4}$ &$7\times 10^{\mbox{-}9}$ &0.5 &1 &1 &11 \\
andes &$7\times 10^{\mbox{-}4}$ (4) &$9\times 10^{\mbox{-}6}$ (3) &$1\times 10^{\mbox{-}5}$ (2) &$3\times 10^{\mbox{-}15}$ (1) &$8\times 10^{\mbox{-}5}$ &$9\times 10^{\mbox{-}7}$ &$1\times 10^{\mbox{-}6}$ &$3\times 10^{\mbox{-}16}$ &0.2 &0.3 &0.4 &2 \\
barley &- (-) &- (-) &$7\times 10^{\mbox{-}4}$ (2) &$7\times 10^{\mbox{-}15}$ (1) &- &- &$4\times 10^{\mbox{-}5}$ &$5\times 10^{\mbox{-}16}$ &- &- &0.1 &0.2 \\
munin1 &0.142 (4) &0.104 (5) &0.017 (4) &$6\times 10^{\mbox{-}4}$ (2) &0.009 &0.006 &0.002 &$5\times 10^{\mbox{-}5}$ &0.2 &0.2 &0.2 &1 \\
munin3 &0.041 (3) &0.005 (2) &$5\times 10^{\mbox{-}4}$ (2) &$2\times 10^{\mbox{-}15}$ (1) &0.002 &$4\times 10^{\mbox{-}4}$ &$4\times 10^{\mbox{-}5}$ &$1\times 10^{\mbox{-}16}$ &1 &1 &1 &2 \\
munin4 &0.088 (4) &0.055 (3) &$2\times 10^{\mbox{-}4}$ (2) &$2\times 10^{\mbox{-}15}$ (1) &0.004 &0.002 &$5\times 10^{\mbox{-}6}$ &$2\times 10^{\mbox{-}16}$ &1 &1 &1 &1 \\
diabetes &- (-) &0.043 (24) &0.049 (23) &$7\times 10^{\mbox{-}4}$ (11) &- &0.01 &0.005 &$5\times 10^{\mbox{-}5}$ &- &1 &1 &4 \\\midrule
\rowcolor{gray!30} \textbf{Average} &\textbf{0.122} &\textbf{0.077} &\textbf{0.030} &\textbf{0.008} &\textbf{0.026} &\textbf{0.013} &\textbf{0.004} &\textbf{0.001} & & & & \\
	\bottomrule
\end{tabular}%
}
\end{table}

==> tables/cmpRuntimePosteriorMAR.tex <==
\begin{table}[!htp]\centering
\caption{Comparison of runtime required for finding posterior marginals with different techniques}{\label{tab:runtimePostMAR}}
\scriptsize
\resizebox{!}{0.25\paperheight}{%
	%\begin{tabular}{lrrrrrrrr}\toprule
	\begin{tabular}{ccccccccc}\toprule
		\textbf{} &\textbf{JTREE} &\textbf{ACE} &\multicolumn{5}{c}{} \\\cmidrule{2-8}
		\textbf{Benchmark} &\textbf{DSDL167} &\textbf{ESL107} &\textbf{WMB} &\textbf{IJGP} &\textbf{FBP} &\textbf{Proposed (with collapse)} &\textbf{Proposed (without collapse)}\\\midrule
BN\_101 &\textbf{y} &\textbf{y} &2 &3 &0.0 &1 &1 \\
BN\_103 &\textbf{y} &\textbf{y} &28 &34 &0.0 &2 &3 \\
BN\_105 &\textbf{y} &\textbf{y} &50 &49 &22.4 &11 &13 \\
BN\_107 &\textbf{y} &\textbf{y} &168 &139 &365.4 &12 &14 \\
BN\_109 &\textbf{y} &\textbf{y} &39 &38 &301.1 &11 &13 \\
BN\_111 &\textbf{y} &\textbf{y} &34 &34 &208.5 &8 &8 \\
BN\_113 &\textbf{y} &\textbf{y} &150 &119 &715.2 &12 &14 \\
BN\_115 &\textbf{y} &\textbf{y} &22 &21 &69.8 &6 &8 \\
BN\_117 &\textbf{y} &\textbf{y} &30 &30 &35.1 &7 &8 \\
BN\_119 &\textbf{y} &\textbf{y} &19 &18 &14.1 &4 &5 \\
BN\_121 &\textbf{y} &\textbf{y} &20 &20 &47.5 &5 &5 \\
BN\_123 &\textbf{y} &\textbf{y} &25 &24 &12.3 &6 &7 \\
BN\_125 &\textbf{y} &\textbf{y} &16 &17 &44.5 &4 &5 \\
BN\_126 &\textbf{n} &\textbf{n} &355 &217 &0.1 &13 &13 \\
BN\_127 &\textbf{n} &\textbf{n} &399 &226 &0.1 &13 &13 \\
BN\_128 &\textbf{n} &\textbf{n} &469 &258 &0.1 &12 &14 \\
BN\_129 &\textbf{n} &\textbf{n} &336 &243 &1.0 &9 &14 \\
BN\_130 &\textbf{n} &\textbf{n} &410 &256 &0.1 &11 &12 \\
BN\_131 &\textbf{n} &\textbf{n} &379 &225 &0.1 &12 &12 \\
BN\_132 &\textbf{n} &\textbf{n} &411 &266 &0.2 &10 &12 \\
BN\_133 &\textbf{n} &\textbf{n} &418 &255 &0.1 &12 &15 \\
BN\_134 &\textbf{n} &\textbf{n} &415 &260 &0.1 &11 &13 \\
BN\_17 &\textbf{n} &\textbf{n} &514 &451 &0.7 &9 &14 \\
BN\_19 &\textbf{n} &\textbf{n} &569 &436 &0.3 &13 &19 \\
BN\_21 &\textbf{y} &\textbf{n} &167 &120 &7.9 &underflow &underflow \\
BN\_23 &\textbf{y} &\textbf{y} &18 &11 &7.1 &4 &5 \\
BN\_25 &\textbf{y} &\textbf{y} &43 &9 &8.4 &3 &3 \\
BN\_27 &\textbf{y} &\textbf{n} &25 &17 &12.9 &underflow &underflow \\
BN\_29 &\textbf{y} &\textbf{y} &3 &3 &3.2 &1 &1 \\
BN\_31 &\textbf{n} &\textbf{y} &438 &390 &0.1 &197 &286 \\
BN\_33 &\textbf{n} &\textbf{y} &579 &474 &0.2 &352 &403 \\
BN\_35 &\textbf{n} &\textbf{y} &492 &442 &87.7 &306 &383 \\
BN\_37 &\textbf{n} &\textbf{y} &549 &500 &91.3 &273 &402 \\
BN\_39 &\textbf{n} &\textbf{y} &491 &435 &84.0 &311 &369 \\
BN\_41 &\textbf{n} &\textbf{y} &510 &475 &0.1 &325 &430 \\
BN\_48 &\textbf{n} &\textbf{y} &647 &508 &0.5 &354 &602 \\
BN\_50 &\textbf{n} &\textbf{y} &734 &510 &0.3 &390 &424 \\
BN\_52 &\textbf{n} &\textbf{y} &590 &498 &0.4 &409 &579 \\
BN\_54 &\textbf{n} &\textbf{y} &415 &293 &0.1 &176 &260 \\
BN\_56 &\textbf{n} &\textbf{y} &447 &319 &0.0 &254 &408 \\
BN\_58 &\textbf{n} &\textbf{y} &457 &335 &0.0 &157 &244 \\
BN\_60 &\textbf{n} &\textbf{y} &551 &376 &0.3 &237 &237 \\
BN\_62 &\textbf{n} &\textbf{y} &680 &542 &0.1 &321 &565 \\
BN\_64 &\textbf{n} &\textbf{y} &578 &325 &0.1 &243 &314 \\
BN\_66 &\textbf{n} &\textbf{y} &423 &322 &0.0 &156 &326 \\
BN\_68 &\textbf{n} &\textbf{y} &382 &209 &0.0 &170 &316 \\
BN\_79 &\textbf{y} &\textbf{y} &0 &0 &0.0 &0 &0 \\
BN\_81 &\textbf{y} &\textbf{y} &1 &1 &0.6 &0 &0 \\
BN\_83 &\textbf{y} &\textbf{y} &3 &4 &1.5 &1 &1 \\
BN\_85 &\textbf{y} &\textbf{y} &4 &3 &1.6 &1 &1 \\
BN\_87 &\textbf{y} &\textbf{y} &242 &156 &28.0 &6 &6 \\
BN\_89 &\textbf{y} &\textbf{y} &8 &8 &55.6 &2 &3 \\
BN\_91 &\textbf{y} &\textbf{y} &114 &81 &25.9 &6 &7 \\
BN\_93 &\textbf{y} &\textbf{y} &17 &14 &44.7 &6 &6 \\
BN\_95 &\textbf{y} &\textbf{y} &5 &5 &0.0 &0 &0 \\
BN\_97 &\textbf{y} &\textbf{y} &6 &8 &0.0 &0 &0 \\
BN\_99 &\textbf{y} &\textbf{y} &18 &14 &0.0 &1 &1 \\
\bottomrule
\end{tabular}%
}
\end{table}
\begin{table}[!htp]\centering
\caption{Runtime(Contd.)}
\resizebox{!}{0.3\paperheight}{%
	%\begin{tabular}{lrrrrrrrr}\toprule
	\begin{tabular}{ccccccccc}\toprule
		\textbf{} &\textbf{JTREE} &\textbf{ACE} &\multicolumn{5}{c}{} \\\cmidrule{2-8}
		\textbf{Benchmark} &\textbf{DSDL167} &\textbf{ESL107} &\textbf{WMB} &\textbf{IJGP} &\textbf{FBP} &\textbf{Proposed (with collapse)} &\textbf{Proposed (without collapse)}\\\midrule
BN\_0 & &\textbf{y} &0 &0 &0.0 &0 &0 \\
BN\_1 & &\textbf{y} &3 &3 &0.0 &3 &3 \\
BN\_10 & &\textbf{y} &0 &0 &0.0 &0 &0 \\
BN\_11 & &\textbf{y} &1 &1 &0.0 &1 &1 \\
BN\_14 & &\textbf{y} &63 &26 &0.0 &5 &6 \\
BN\_2 & &\textbf{y} &69 &41 &0.0 &0 &0 \\
BN\_28 & &\textbf{y} &3 &3 &3.0 &1 &1 \\
BN\_3 & &\textbf{y} &0 &0 &0.0 &0 &0 \\
BN\_30 & &\textbf{y} &576 &341 &0.1 &228 &250 \\
BN\_32 & &\textbf{y} &606 &510 &0.2 &290 &430 \\
BN\_34 & &\textbf{y} &707 &478 &84.3 &320 &496 \\
BN\_36 & &\textbf{y} &670 &455 &89.3 &338 &381 \\
BN\_38 & &\textbf{y} &594 &414 &85.3 &278 &391 \\
BN\_4 & &\textbf{y} &0 &0 &0.0 &0 &0 \\
BN\_40 & &\textbf{y} &626 &439 &0.1 &307 &362 \\
BN\_42 & &\textbf{y} &68 &64 &26.4 &125 &39 \\
BN\_43 & &\textbf{y} &129 &89 &35.6 &85 &116 \\
BN\_44 & &\textbf{y} &89 &71 &0.1 &69 &66 \\
BN\_45 & &\textbf{y} &89 &82 &29.8 &55 &46 \\
BN\_46 & &\textbf{y} &114 &89 &0.0 &48 &35 \\
BN\_47 & &\textbf{y} &660 &525 &0.5 &390 &586 \\
BN\_49 & &\textbf{y} &778 &564 &0.3 &321 &572 \\
BN\_5 & &\textbf{y} &0 &0 &0.0 &0 &0 \\
BN\_51 & &\textbf{y} &701 &492 &0.4 &342 &435 \\
BN\_53 & &\textbf{y} &477 &333 &0.0 &198 &258 \\
BN\_55 & &\textbf{y} &525 &348 &0.0 &167 &311 \\
BN\_57 & &\textbf{y} &561 &324 &0.0 &190 &223 \\
BN\_59 & &\textbf{y} &561 &392 &0.3 &172 &186 \\
BN\_6 & &\textbf{y} &0 &0 &0.0 &0 &0 \\
BN\_61 & &\textbf{y} &765 &497 &0.2 &449 &562 \\
BN\_63 & &\textbf{y} &519 &477 &0.1 &213 &329 \\
BN\_65 & &\textbf{y} &474 &345 &0.0 &140 &189 \\
BN\_67 & &\textbf{y} &438 &305 &0.0 &171 &318 \\
BN\_7 & &\textbf{y} &1 &1 &0.0 &1 &1 \\
BN\_78 & &\textbf{y} &0 &0 &0.0 &0 &0 \\
BN\_8 & &\textbf{y} &101 &92 &0.0 &5 &5 \\
BN\_80 & &\textbf{y} &1 &1 &0.6 &0 &0 \\
BN\_82 & &\textbf{y} &4 &3 &1.5 &1 &1 \\
BN\_84 & &\textbf{y} &5 &4 &2.2 &1 &1 \\
BN\_86 & &\textbf{y} &213 &162 &19.4 &2 &3 \\
BN\_88 & &\textbf{y} &8 &9 &19.6 &2 &2 \\
BN\_9 & &\textbf{y} &67 &60 &0.0 &5 &6 \\
BN\_90 & &\textbf{y} &109 &95 &103.0 &5 &6 \\
BN\_92 & &\textbf{y} &18 &15 &128.2 &7 &7 \\
BN\_22 & &\textbf{y} &19 &11 &4.8 &4 &4 \\
BN\_24 & &\textbf{y} &9 &7 &8.5 &3 &3 \\
BN\_12 & &\textbf{n} &106 &86 &0.0 &1 &1 \\
BN\_13 & &\textbf{n} &129 &90 &0.0 &1 &1 \\
BN\_15 & &\textbf{n} &173 &93 &0.0 &1 &2 \\
BN\_16 & &\textbf{n} &519 &344 &0.7 &11 &13 \\
BN\_20 & &\textbf{n} &176 &122 &5.6 &underflow &underflow \\
BN\_26 & &\textbf{n} &26 &18 &11.5 &underflow &underflow \\
BN\_69 & &\textbf{n} &OOM &OOM &101.5 &6 &8 \\
BN\_70 & &\textbf{n} &OOM &OOM &1.2 &53 &76 \\
BN\_71 & &\textbf{n} &OOM &OOM &1.0 &26 &29 \\
BN\_72 & &\textbf{n} &OOM &OOM &871.9 &51 &57 \\
BN\_73 & &\textbf{n} &OOM &OOM &0.8 &48 &Not possible to continue CT \\
BN\_74 & &\textbf{n} &OOM &OOM &176.5 &4 &5 \\
BN\_75 & &\textbf{n} &OOM &OOM &1.2 &56 &41 \\
BN\_76 & &\textbf{n} &OOM &OOM &1040.0 &36 &33 \\
BN\_77 & &\textbf{n} &OOM &OOM &0.9 &6 &7 \\
\bottomrule
\end{tabular}%
}
\end{table}

==> tables/compareSimplify.tex <==
% !TeX spellcheck = en_US
\begin{table}[!htbp]\centering
\caption{Impact of simplification on the errors in $PR$ and $MAR_e$ inferred using BIA with $mcs_p=20,~mcs_{im}=15$. We report check accuracy for marginals upto three decimal places. The error is reported as 0 when it is $<10^{-16}$.\\
	\textcolor{red}{Different formats and precision bits for each column (<0.001 in one and $10^-7$ in another). Should we move difference in PR to a different table?}}
\label{tab:compareSimplify}
\scriptsize
\resizebox{!}{0.35\paperheight}{
	\begin{tabular}{|c|cc|cc|cc|}\toprule
	\multirow{2}{*}{\textbf{Benchmark}} &\multicolumn{2}{c|}{$\mathbf{\Delta_{BIA}}$} &\multicolumn{2}{c|}{\textbf{Maximum Error (\#Partitions)}} &\multicolumn{2}{c|}{\textbf{RMSE}} \\\cmidrule{2-7}
	&\textbf{w/ simplify} &\textbf{w/o simplify } &\textbf{w/ simplify} &\textbf{w/o simplify} &\textbf{w/ simplify} &\textbf{w/o simplify} \\\midrule
BN\_105 &-$9 \times 10^{\mbox{-}7}$ &-$9 \times 10^{\mbox{-}7}$ &0 (1) &0 (1) &0 &0 \\
BN\_107 &-$2 \times 10^{\mbox{-}7}$ &-$2 \times 10^{\mbox{-}7}$ &0 (1) &0.021 (6) &0 &0.004 \\
BN\_109 &$3 \times 10^{\mbox{-}7}$ &-0.004 &0 (1) &0.013 (2) &0 &0.004 \\
BN\_111 &-$2 \times 10^{\mbox{-}7}$ &-$2 \times 10^{\mbox{-}7}$ &0 (1) &0 (1) &0 &0 \\
BN\_113 &0 &0 &0 (1) &<0.001 (5) &0 &<0.001 \\
BN\_14 &$5 \times 10^{\mbox{-}4}$ &$5 \times 10^{\mbox{-}4}$ &0.012 (3) &0.012 (3) &0.002 &0.002 \\
BN\_2 &$4 \times 10^{\mbox{-}7}$ &$4 \times 10^{\mbox{-}7}$ &0.001 (2) &0.001 (2) &<0.001 &<0.001 \\
BN\_22 &0 &0 &0 (1) &0 (1) &0 &0 \\
BN\_23 &0 &0 &0 (1) &0 (1) &0 &0 \\
BN\_24 &-$7 \times 10^{\mbox{-}7}$ &-$7 \times 10^{\mbox{-}7}$ &0 (1) &0 (1) &0 &0 \\
BN\_25 &-$7 \times 10^{\mbox{-}7}$ &-$7 \times 10^{\mbox{-}7}$ &0 (1) &0 (1) &0 &0 \\
BN\_30 &-$4 \times 10^{\mbox{-}7}$ &-$7 \times 10^{\mbox{-}5}$ &0 (1) &0.329 (10) &0 &0.029 \\
BN\_31 &-$4 \times 10^{\mbox{-}7}$ &$3 \times 10^{\mbox{-}4}$ &0 (1) &0.350 (11) &0 &0.025 \\
BN\_32 &-$2 \times 10^{\mbox{-}7}$ &0.002 &0 (1) &0.106 (16) &0 &0.013 \\
BN\_33 &-$2 \times 10^{\mbox{-}7}$ &0.010 &0 (1) &0.143 (12) &0 &0.006 \\
BN\_34 &$1 \times 10^{\mbox{-}7}$ &-0.009 &0 (1) &0.086 (15) &0 &0.006 \\
BN\_35 &$1 \times 10^{\mbox{-}7}$ &$1 \times 10^{\mbox{-}7}$ &0 (1) &0.084 (14) &0 &0.006 \\
BN\_36 &$2 \times 10^{\mbox{-}7}$ &$2 \times 10^{\mbox{-}7}$ &0 (1) &0.122 (13) &0 &0.009 \\
BN\_37 &$2 \times 10^{\mbox{-}7}$ &0.060 &0 (1) &0.145 (15) &0 &0.011 \\
BN\_38 &0 &0 &0 (1) &0.035 (14) &0 &0.004 \\
BN\_39 &0 &$3 \times 10^{\mbox{-}6}$ &0 (1) &0.041 (12) &0 &0.003 \\
BN\_40 &$7 \times 10^{\mbox{-}8}$ &$7 \times 10^{\mbox{-}8}$ &0 (1) &0.094 (12) &0 &0.006 \\
BN\_41 &$7 \times 10^{\mbox{-}8}$ &$7 \times 10^{\mbox{-}8}$ &0 (1) &0.055 (13) &0 &0.007 \\
BN\_42 &-$5 \times 10^{\mbox{-}7}$ &0.030 &0.052 (4) &0.132 (12) &0.008 &0.031 \\
BN\_43 &-$4 \times 10^{\mbox{-}5}$ &-$2 \times 10^{\mbox{-}7}$ &0.003 (3) &0.093 (7) &<0.001 &0.014 \\
BN\_44 &-$8 \times 10^{\mbox{-}7}$ &-$7 \times 10^{\mbox{-}4}$ &0 (1) &0.038 (5) &0 &0.009 \\
BN\_45 &$1 \times 10^{\mbox{-}6}$ &$5 \times 10^{\mbox{-}5}$ &<0.001 (3) &0.094 (7) &<0.001 &0.013 \\
BN\_46 &$7 \times 10^{\mbox{-}7}$ &$7 \times 10^{\mbox{-}7}$ &0 (1) &<0.001 (4) &0 &<0.001 \\
BN\_47 &-$5 \times 10^{\mbox{-}8}$ &-$5 \times 10^{\mbox{-}8}$ &<0.001 (3) &0.118 (9) &<0.001 &0.011 \\
BN\_48 &-$5 \times 10^{\mbox{-}8}$ &-$5 \times 10^{\mbox{-}8}$ &<0.001 (3) &0.118 (7) &<0.001 &0.015 \\
BN\_49 &$7 \times 10^{\mbox{-}7}$ &$7 \times 10^{\mbox{-}7}$ &0 (1) &0.029 (10) &0 &0.008 \\
BN\_50 &$7 \times 10^{\mbox{-}7}$ &$7 \times 10^{\mbox{-}7}$ &0 (1) &0.010 (9) &0 &0.001 \\
BN\_51 &$2 \times 10^{\mbox{-}7}$ &-0.030 &0 (1) &0.357 (8) &0 &0.048 \\
BN\_52 &$2 \times 10^{\mbox{-}7}$ &-0.003 &0 (1) &0.357 (8) &0 &0.059 \\
BN\_53 &$2 \times 10^{\mbox{-}7}$ &0.010 &0.020 (7) &0.064 (11) &0.001 &0.009 \\
BN\_54 &$7 \times 10^{\mbox{-}6}$ &$2 \times 10^{\mbox{-}7}$ &0.015 (7) &0.034 (9) &0.001 &0.008 \\
BN\_55 &$7 \times 10^{\mbox{-}7}$ &$7 \times 10^{\mbox{-}7}$ &0.006 (3) &0.029 (11) &0.001 &0.004 \\
BN\_56 &$7 \times 10^{\mbox{-}7}$ &0.030 &0.006 (3) &0.121 (11) &0.001 &0.038 \\
BN\_57 &$2 \times 10^{\mbox{-}6}$ &$2 \times 10^{\mbox{-}6}$ &0.005 (2) &0.146 (10) &<0.001 &0.01 \\
BN\_58 &$2 \times 10^{\mbox{-}6}$ &$2 \times 10^{\mbox{-}6}$ &<0.001 (2) &0.146 (10) &<0.001 &0.009 \\
BN\_59 &$1 \times 10^{\mbox{-}7}$ &$1 \times 10^{\mbox{-}7}$ &0.054 (6) &0.339 (11) &0.004 &0.078 \\
BN\_60 &$1 \times 10^{\mbox{-}7}$ &$1 \times 10^{\mbox{-}7}$ &0.054 (5) &0.402 (11) &0.004 &0.083 \\
BN\_61 &$1 \times 10^{\mbox{-}6}$ &-0.030 &0 (1) &0.167 (9) &0 &0.025 \\
BN\_62 &$1 \times 10^{\mbox{-}6}$ &$1 \times 10^{\mbox{-}6}$ &0 (1) &0.142 (10) &0 &0.012 \\
BN\_63 &-$4 \times 10^{\mbox{-}5}$ &-0.001 &0.007 (7) &0.074 (10) &0.001 &0.01 \\
BN\_64 &-$1 \times 10^{\mbox{-}5}$ &-0.003 &0.009 (8) &0.110 (9) &0.001 &0.012 \\
BN\_65 &$5 \times 10^{\mbox{-}8}$ &-0.003 &0.033 (7) &0.108 (9) &0.003 &0.01 \\
BN\_66 &$5 \times 10^{\mbox{-}8}$ &0.001 &0.064 (7) &0.088 (13) &0.005 &0.009 \\
BN\_67 &-$5 \times 10^{\mbox{-}5}$ &-0.010 &0.040 (7) &0.113 (11) &0.005 &0.015 \\
BN\_68 &-$1 \times 10^{\mbox{-}5}$ &-0.010 &0.021 (7) &0.073 (10) &0.002 &0.013 \\
BN\_8 &$4 \times 10^{\mbox{-}6}$ &$4 \times 10^{\mbox{-}6}$ &0.002 (4) &0.002 (4) &<0.001 &<0.001 \\
BN\_86 &-$4 \times 10^{\mbox{-}7}$ &-$4 \times 10^{\mbox{-}7}$ &<0.001 (2) &<0.001 (2) &<0.001 &<0.001 \\
BN\_87 &-$4 \times 10^{\mbox{-}7}$ &-$4 \times 10^{\mbox{-}7}$ &<0.001 (2) &<0.001 (2) &<0.001 &<0.001 \\
BN\_9 &-$3 \times 10^{\mbox{-}4}$ &-$3 \times 10^{\mbox{-}4}$ &0.019 (4) &0.019 (4) &0.002 &0.002 \\
BN\_90 &-$1 \times 10^{\mbox{-}7}$ &-$1 \times 10^{\mbox{-}7}$ &<0.001 (3) &<0.001 (2) &<0.001 &<0.001 \\
BN\_91 &-$1 \times 10^{\mbox{-}7}$ &-$1 \times 10^{\mbox{-}7}$ &<0.001 (3) &<0.001 (3) &<0.001 &<0.001 \\
BN\_95 &-$3 \times 10^{\mbox{-}7}$ &-$3 \times 10^{\mbox{-}7}$ &0.006 (2) &0.006 (2) &0.001 &0.001 \\
\rowcolor{gray!30}	\textbf{Mean} &$\mathbf{1 \times 10^{\mbox{-}6}}$ &$\mathbf{7 \times 10^{\mbox{-}4}}$ &\textbf{0.091} &\textbf{0.058} &\textbf{0.001} &\textbf{0.012} \\
\bottomrule
\end{tabular}%
}
\end{table}

==> tables/incrVStriangulate.tex <==
% !TeX spellcheck = en_US
\begin{table}[!htp]\centering
\caption{Comparison of the maximum clique size obtained after incremental construction ($mcs_i$) of the first CTF with that obtained after full compilation of the corresponding BN subgraph ($mcs_{f}$). The number of variables in the CTF are indicated in column $\#Var.$ For each benchmark, we show results for CTFs obtained using different clique size constraints. Entries are marked with dash if the maximum factor size of CPDs $>mcs_p$.  $\Delta=mcs_i-mcs_f$.}\label{tab:incrVStriang}
\scriptsize
\setlength\tabcolsep{2pt}
\resizebox{\textwidth}{!}{%
	\begin{tabular}{|c|ccc|>{\columncolor{gray!30}}c|ccc|>{\columncolor{gray!30}}c|ccc|>{\columncolor{gray!30}}c|ccc|>{\columncolor{gray!30}}c|}\toprule
		\multirow{2}{*}{\textbf{Network}} &\multicolumn{4}{c|}{$\mathbf{mcs_p=10}$} &\multicolumn{4}{c|}{$\mathbf{mcs_p=15}$} &\multicolumn{4}{c|}{$\mathbf{mcs_p=20}$} &\multicolumn{4}{c|}{$\mathbf{mcs_p=25}$} \\\cmidrule{2-17}
&\textbf{\#Var.} &$\mathbf{mcs_i}$ &$\mathbf{mcs_{f}}$ &$\mathbf{\Delta}$ &\textbf{\#Var.} &$\mathbf{mcs_i}$ &$\mathbf{mcs_{f}}$ &$\mathbf{\Delta}$ &\textbf{\#Var.} &$\mathbf{mcs_i}$ &$\mathbf{mcs_{f}}$ &$\mathbf{\Delta}$ &\textbf{\#Var.} &$\mathbf{mcs_i}$ &$\mathbf{mcs_{f}}$ &$\mathbf{\Delta}$ \\\midrule
BN\_55 &217 &10 &10 &0 &254 &15 &15 &0 &294 &20 &20 &0 &309 &25 &23 &2 \\
BN\_62 &173 &10 &10 &0 &343 &14 &14 &0 &455 &20 &19 &1 &517 &24 &23 &1 \\
BN\_51 &183 &10 &10 &0 &357 &15 &15 &0 &467 &20 &19 &1 &541 &25 &25 &0 \\
BN\_21 &- &- &- &- &624 &13.2 &15.2 &-1.9 &627 &17.2 &16.2 &1 &2832 &20.2 &21.2 &-1 \\
mastermind\_03\_08\_03-0010 &376 &10 &11 &-1 &579 &15 &16 &-1 &743 &20 &20 &0 &817 &22 &19 &3 \\
mastermind\_03\_08\_04-0010 &372 &10 &10 &0 &748 &15 &15 &0 &1051 &20 &21 &-1 &1204 &25 &24 &1 \\
mastermind\_03\_08\_05-0010 &339 &6 &6 &0 &591 &15 &15 &0 &1135 &18 &18 &0 &1503 &25 &24 &1 \\
blockmap\_15\_01-0006 &1177 &10 &11 &-1 &1873 &15 &15 &0 &3851 &20 &21 &-1 &5001 &25 &24 &1 \\
blockmap\_10\_01-0005 &477 &10 &10 &0 &1076 &15 &16 &-1 &1602 &20 &20 &0 &2165 &25 &24 &1 \\
90-23-5 &171 &10 &10 &0 &206 &15 &12 &3 &235 &20 &14 &6 &268 &24 &15 &9 \\
90-42-5 &292 &10 &10 &0 &399 &15 &13 &2 &531 &20 &16 &4 &583 &25 &18 &7 \\
50-18-5 &131 &10 &10 &0 &194 &15 &13 &2 &229 &20 &18 &2 &251 &24 &22 &2 \\
90-50-5 &517 &10 &9 &1 &598 &15 &13 &2 &740 &20 &18 &2 &848 &25 &19 &6 \\
munin1 &68 &9.2 &9.2 &0 &74 &13.3 &13.3 &0 &80 &17.6 &17.6 &0 &129 &24 &25 &-1 \\
diabetes &- &- &- &- &186 &13.6 &13.6 &0 &192 &19.2 &18.9 &0.4 &196 &22.7 &18.2 &4.5 \\
munin4 &283 &9.6 &9.6 &0 &301 &13.9 &14.2 &-0.3 &634 &19.6 &21.4 &-1.8 &642 &20.4 &21.4 &-1 \\
\rowcolor{gray!30}$\mathbf{\Delta_{Mean}}$ & & & &{\it \textbf{-0.07}} & & & &{\it \textbf{0.3}} & & & &{\it \textbf{0.85}} & & & &{\it \textbf{2.22}} \\
\bottomrule
\end{tabular}%
}
\end{table}


==> tables/postmar.bnuai.ace.abs.tex <==
% !TeX spellcheck = en_US

\begin{table}[!htp]\centering
	\caption{Comparison of absolute value of the maximum error and RMSE in $MAR_e$ for BN\_UAI benchmarks. For IBIA, errors are reported for two sets of clique size constraints: $mcs_p=20, ~mcs_{im}=15$ and $mcs_p=15, ~mcs_{im}=10$. Entries are marked with `-' where inference fails. For consistency in precision across algorithms, the error is reported as zero if accurate to three decimal places.}
	\label{tab:postmar.bnuai.ace.abs}
	\scriptsize
	\setlength\tabcolsep{2pt}
	\resizebox{!}{0.32\paperheight}{%
	%\begin{tabular}{l|rrrrr|rrrrr|rrrrrrr}\toprule
	\begin{tabular}{|c|ccc>{\columncolor{gray!30}}c>{\columncolor{gray!30}}c|ccc>{\columncolor{gray!30}}c>{\columncolor{gray!30}}c|}\toprule
		\multirow{3}{*}{\textbf{Benchmark}} &\multicolumn{5}{c|}{\textbf{Maximum Error}} &\multicolumn{5}{c|}{\textbf{RMSE}} \\ \cline{2-11}
		&\multirow{2}{*}{\textbf{FBP}}  & \multirow{2}{*}{\textbf{WMB}} &\multirow{2}{*}{\textbf{IJGP}} &\textbf{IBIA} &\textbf{IBIA} &\multirow{2}{*}{\textbf{FBP}} &\multirow{2}{*}{\textbf{WMB}} &\multirow{2}{*}{\textbf{IJGP}} &\textbf{IBIA} &\textbf{IBIA} \\
		&&&&$\mathbf{mcs_p=20}$&$\mathbf{mcs_p=15}$&&&&$\mathbf{mcs_p=20}$&$\mathbf{mcs_p=15}$ \\\midrule
BN\_105 &0.411 &0 &0 &0 &0 &0.15 &0 &0 &0 &0 \\
BN\_107 &0.149 &0.337 &0.194 &0 &0 &0.042 &0.077 &0.056 &0 &0 \\
BN\_109 &0.272 &0 &0 &0 &0 &0.111 &0 &0 &0 &0 \\
BN\_111 &0.344 &0 &0 &0 &0 &0.117 &0 &0 &0 &0 \\
BN\_113 &0.212 &0 &0.489 &0 &0 &0.088 &0 &0.184 &0 &0 \\
BN\_14 &0.019 &0.01 &0.641 &0.012 &0.012 &0.003 &0.002 &0.142 &0.002 &0.003 \\
BN\_2 &0.015 &0.033 &0.53 &0.001 &0.001 &0.003 &0.009 &0.222 &0 &0.001 \\
BN\_22 &0.397 &0 &0 &0 &0 &0.017 &0 &0 &0 &0.002 \\
BN\_23 &0.397 &0 &0 &0 &0 &0.017 &0 &0 &0 &0.002 \\
BN\_24 &0.127 &0 &0 &0 &0 &0.016 &0 &0 &0 &0 \\
BN\_25 &0.127 &0 &0 &0 &0 &0.016 &0 &0 &0 &0 \\
BN\_30 &0.515 &0.362 &0.59 &0 &0 &0.077 &0.057 &0.107 &0 &0 \\
BN\_31 &0.515 &0.447 &0.735 &0 &0 &0.077 &0.058 &0.126 &0 &0 \\
BN\_32 &0.622 &0.433 &0.509 &0 &0 &0.114 &0.069 &0.097 &0 &0 \\
BN\_33 &0.622 &0.668 &0.925 &0 &0 &0.114 &0.077 &0.133 &0 &0 \\
BN\_34 &0.952 &0.493 &0.746 &0 &0 &0.146 &0.062 &0.123 &0 &0 \\
BN\_35 &0.952 &0.694 &0.869 &0 &0 &0.141 &0.077 &0.123 &0 &0 \\
BN\_36 &0.719 &0.567 &0.642 &0 &0 &0.103 &0.051 &0.107 &0 &0 \\
BN\_37 &0.719 &0.663 &0.597 &0 &0 &0.103 &0.071 &0.109 &0 &0 \\
BN\_38 &1 &0.567 &0.798 &0 &0 &0.119 &0.071 &0.166 &0 &0 \\
BN\_39 &1 &0.375 &0.689 &0 &0 &0.119 &0.054 &0.133 &0 &0 \\
BN\_40 &0.817 &0.395 &0.629 &0 &0 &0.114 &0.051 &0.080 &0 &0 \\
BN\_41 &0.817 &0.314 &0.536 &0 &0 &0.114 &0.044 &0.085 &0 &0 \\
BN\_42 &0.261 &0.049 &0.831 &0.052 &0.052 &0.043 &0.011 &0.214 &0.008 &0.015 \\
BN\_43 &0.286 &0.187 &0.658 &0.003 &0.003 &0.067 &0.039 &0.157 &0 &0.006 \\
BN\_44 &0.193 &0.08 &0.596 &0 &0 &0.039 &0.022 &0.210 &0 &0.004 \\
BN\_45 &0.332 &0.059 &0.469 &0 &0 &0.041 &0.013 &0.111 &0 &0.001 \\
BN\_46 &0.026 &0.3 &0.5 &0 &0 &0.003 &0.044 &0.164 &0 &0 \\
BN\_47 &0.307 &0.53 &0.765 &0 &0 &0.1 &0.135 &0.203 &0 &0.003 \\
BN\_48 &0.307 &0.767 &- &0 &0 &0.1 &0.168 &- &0 &0.005 \\
BN\_49 &0.179 &0.409 &0.59 &0 &0 &0.051 &0.098 &0.162 &0 &0 \\
BN\_50 &0.179 &0.378 &0.59 &0 &0 &0.051 &0.083 &0.163 &0 &0 \\
BN\_51 &0.204 &0.587 &- &0 &0 &0.066 &0.186 &- &0 &0 \\
BN\_52 &0.204 &0.636 &- &0 &0 &0.066 &0.213 &- &0 &0 \\
BN\_53 &0.183 &0.421 &- &0.02 &0.02 &0.044 &0.138 &- &0.001 &0.009 \\
BN\_54 &0.183 &0.387 &0.871 &0.015 &0.015 &0.044 &0.132 &0.300 &0.001 &0.004 \\
BN\_55 &0.191 &0.525 &0.875 &0.006 &0.006 &0.038 &0.14 &0.244 &0.001 &0.001 \\
BN\_56 &0.191 &0.426 &0.858 &0.006 &0.006 &0.038 &0.137 &0.243 &0.001 &0.001 \\
BN\_57 &0.179 &0.362 &- &0.005 &0.005 &0.026 &0.091 &- &0 &0.002 \\
BN\_58 &0.179 &0.311 &0.806 &0 &0 &0.026 &0.094 &0.301 &0 &0.002 \\
BN\_59 &0.5 &0.613 &- &0.054 &0.054 &0.164 &0.153 &- &0.004 &0.125 \\
BN\_60 &0.5 &0.513 &- &0.054 &0.054 &0.164 &0.15 &- &0.004 &0.122 \\
BN\_61 &0.105 &0.148 &- &0 &0 &0.016 &0.028 &- &0 &0 \\
BN\_62 &0.105 &0.151 &- &0 &0 &0.016 &0.033 &- &0 &0 \\
BN\_63 &0.184 &0.574 &0.884 &0.007 &0.007 &0.033 &0.161 &0.260 &0.001 &0.006 \\
BN\_64 &0.184 &0.58 &0.924 &0.009 &0.009 &0.033 &0.16 &0.312 &0.001 &0.005 \\
BN\_65 &0.496 &0.649 &0.749 &0.033 &0.033 &0.071 &0.202 &0.195 &0.003 &0.006 \\
BN\_66 &0.496 &0.726 &0.96 &0.064 &0.064 &0.071 &0.212 &0.233 &0.005 &0.005 \\
BN\_67 &0.086 &0.717 &0.876 &0.04 &0.04 &0.013 &0.22 &0.222 &0.005 &0.003 \\
BN\_68 &0.086 &0.638 &0.83 &0.021 &0.021 &0.013 &0.207 &0.191 &0.002 &0.003 \\
BN\_8 &0.031 &0.054 &0.556 &0.002 &0.002 &0.004 &0.009 &0.251 &0 &0.003 \\
BN\_86 &0 &0 &0.273 &0 &- &0 &0 &0.014 &0 &- \\
BN\_87 &0 &0 &0.5 &0 &- &0 &0 &0.030 &0 &- \\
BN\_9 &0.025 &0.055 &0.624 &0.019 &0.019 &0.003 &0.007 &0.207 &0.002 &0.002 \\
BN\_90 &0 &0 &0.357 &0 &- &0 &0 &0.019 &0 &- \\
BN\_91 &0 &0 &0.357 &0 &- &0 &0 &0.019 &0 &- \\
BN\_95 &0.119 &0 &0 &0.006 &0.006 &0.032 &0 &0 &0.001 &0.003 \\ \midrule
\rowcolor{gray!30}{\bf Mean} &{\bf 0.320}  &{\bf 0.319} &{\bf 0.550} &{\bf 0.008} &{\bf 0.037} &{\bf 0.060} &{\bf 0.072} &{\bf 0.134} &{\bf 0.001} &{\bf 0.006} \\
\bottomrule
	\end{tabular}%
	}
%        \vskip 1pt
%        {\footnotesize $^1$As discussed, the error is set to zero if the marginals match to three decimal places}
%{\footnotesize *Values in brackets indicate number of partitions}
\end{table}


==> tables/postmar.bnuai.runtime.tex <==
% !TeX spellcheck = en_US
\begin{table}[!htp]\centering
\caption{Comparion of runtime required (in seconds) to estimate posterior node marginals using different inference algorithms for BN\_UAI. For IBIA, runtimes are reported for two sets of clique size constraints: $mcs_p=20, ~mcs_{im}=15$ and $mcs_p=15, ~mcs_{im}=10$.  Entries are marked with `-' where inference fails.}\label{tab:runtimePosteriorBN}
\scriptsize
\setlength\tabcolsep{3.5pt}
	\resizebox{!}{0.34\paperheight}{%
\begin{tabular}{|c|ccc|c|c|c|>{\columncolor{gray!30}}c>{\columncolor{gray!30}}c|}\toprule
\multirow{2}{*}{\textbf{Benchmark}} &\multicolumn{3}{c|}{\textbf{ACE}} &\multirow{2}{*}{\textbf{FBP}} &\multirow{2}{*}{\textbf{WMB}} &\multirow{2}{*}{\textbf{IJGP}} &\multicolumn{2}{c|}{\textbf{IBIA}} \\\cmidrule{2-4}\cmidrule{8-9}
&\textbf{Compile*} &\textbf{Evaluate} &\textbf{Total} & & & &\textbf{$\mathbf{mcs_p=20}$} &\textbf{$\mathbf{mcs_p=15}$} \\\midrule
BN\_105 &3 &1 &4 &22 &50 &49 &11 &11 \\
BN\_107 &3 &1 &4 &365 &168 &139 &9 &9 \\
BN\_109 &2 &1 &3 &301 &39 &38 &8 &8 \\
BN\_111 &2 &1 &3 &209 &34 &34 &8 &7 \\
BN\_113 &2 &1 &3 &715 &150 &119 &8 &8 \\
BN\_14 &8 &24 &32 &0.01 &63 &26 &3 &1 \\
BN\_2 &6 &20 &26 &0.01 &69 &41 &0.3 &0.4 \\
BN\_22 &3 &1 &4 &5 &19 &11 &5 &47 \\
BN\_23 &5 &2 &7 &7 &18 &11 &5 &40 \\
BN\_24 &2 &1 &3 &8 &9 &7 &4 &4 \\
BN\_25 &4 &2 &6 &8 &43 &9 &4 &4 \\
BN\_30 &0.4 &0.1 &0.5 &0.1 &576 &341 &1 &1 \\
BN\_31 &0.4 &0.1 &0.5 &0.1 &438 &390 &1 &1 \\
BN\_32 &1 &0.1 &1.1 &0.2 &606 &510 &1 &1 \\
BN\_33 &0.5 &0.1 &0.6 &0.2 &579 &474 &1 &1 \\
BN\_34 &0.5 &0.1 &0.6 &84 &707 &478 &1 &1 \\
BN\_35 &0.5 &0.1 &0.6 &88 &492 &442 &1 &1 \\
BN\_36 &0.4 &0.1 &0.5 &89 &670 &455 &1 &1 \\
BN\_37 &0.4 &0.1 &0.5 &91 &549 &500 &1 &1 \\
BN\_38 &0.5 &0.1 &0.6 &85 &594 &414 &1 &1 \\
BN\_39 &0.5 &0.1 &0.6 &84 &491 &435 &1 &1 \\
BN\_40 &0.4 &0.1 &0.5 &0.1 &626 &439 &1 &1 \\
BN\_41 &0.4 &0.1 &0.5 &0.1 &510 &475 &1 &1 \\
BN\_42 &2 &4 &6 &26 &68 &64 &9 &3 \\
BN\_43 &1 &1 &2 &36 &129 &89 &2 &1 \\
BN\_44 &2 &1 &3 &0.1 &89 &71 &0.4 &2 \\
BN\_45 &2 &3 &5 &30 &89 &82 &1 &1 \\
BN\_46 &1 &1 &2 &0.01 &114 &89 &0.3 &0.3 \\
BN\_47 &0.3 &0.1 &0.4 &1 &660 &525 &2 &9 \\
BN\_48 &0.3 &0.1 &0.4 &1 &647 &- &2 &9 \\
BN\_49 &0.3 &0.1 &0.4 &0.3 &778 &564 &1 &2 \\
BN\_50 &0.3 &0.1 &0.4 &0.3 &734 &510 &1 &1 \\
BN\_51 &0.3 &0.1 &0.4 &0.4 &701 &- &1 &1 \\
BN\_52 &0.3 &0.1 &0.4 &0.4 &590 &- &1 &1 \\
BN\_53 &0.4 &0.1 &0.5 &0.05 &477 &- &15 &6 \\
BN\_54 &0.4 &0.1 &0.5 &0.05 &415 &293 &19 &5 \\
BN\_55 &0.3 &0.1 &0.4 &0.05 &525 &348 &6 &1 \\
BN\_56 &0.3 &0.1 &0.4 &0.04 &447 &319 &8 &1 \\
BN\_57 &0.3 &0.1 &0.4 &0.02 &561 &- &1 &0.4 \\
BN\_58 &0.3 &0.1 &0.4 &0.02 &457 &335 &1 &0.4 \\
BN\_59 &0.3 &0.1 &0.4 &0.3 &561 &- &2 &5 \\
BN\_60 &0.3 &0.1 &0.4 &0.3 &551 &- &2 &5 \\
BN\_61 &0.3 &0.1 &0.4 &0.2 &765 &- &1 &1 \\
BN\_62 &0.3 &0.1 &0.4 &0.1 &680 &- &1 &1 \\
BN\_63 &0.5 &0.1 &0.6 &0.1 &519 &477 &40 &12 \\
BN\_64 &1 &0.1 &1.1 &0.1 &578 &325 &42 &11 \\
BN\_65 &1 &0.1 &1.1 &0.03 &474 &345 &4 &2 \\
BN\_66 &0.4 &0.1 &0.5 &0.03 &423 &322 &7 &3 \\
BN\_67 &0.5 &0.1 &0.6 &0.03 &438 &305 &14 &3 \\
BN\_68 &0.5 &0.1 &0.6 &0.03 &382 &209 &7 &3 \\
BN\_8 &42 &131 &173 &0.01 &101 &92 &3 &1 \\
BN\_86 &6 &14 &20 &19 &213 &162 &3 &- \\
BN\_87 &4 &13 &17 &28 &242 &156 &3 &- \\
BN\_9 &36 &113 &149 &0.01 &67 &60 &2 &1 \\
BN\_90 &6 &15 &21 &103 &109 &95 &2 &- \\
BN\_91 &6 &14 &20 &26 &114 &81 &3 &- \\
BN\_95 &1 &4 &5 &0.01 &5 &5 &0.2 &0.2 \\
\bottomrule
\end{tabular}%
}
{\\ \footnotesize *Compilation performed with evidence}
\end{table}


==> tables/pr.bnuai.ace.tex <==
% !TeX spellcheck = en_US
\begin{table}[!htp]\centering
\caption{Exact probability of evidence obtained using the ACE solver ($PR_{ACE}$) and the error in PR estimated using different approximate inference techniques ($\Delta_{Alg}=\log ~PR_{Alg}-\log~PR_{ACE}$) for various BN\_UAI benchmarks. Entries are marked with `-' for testcases where inferred PR is greater than $1$.}\label{tab:pr.bnuai.ace}
\scriptsize
	\resizebox{!}{0.35\paperheight}{%
	\begin{tabular}{|cccc>{\columncolor{gray!30}}c|}\toprule
	\textbf{Benchmark} &\textbf{$\log~PR_{ACE}$} &\textbf{$\Delta_{FBP}$}&\textbf{$\Delta_{WMB}$} &\textbf{$\Delta_{IBIA}$} \\\bottomrule
BN\_105 &-0.83 &0.12 &$8\times10^{\mbox{-}8}$ &-$9\times10^{\mbox{-}7}$ \\
BN\_107 &-1.15 &-0.07 &0.22 &-$2\times10^{\mbox{-}7}$ \\
BN\_109 &-1.89 &-0.20 &$1\times10^{\mbox{-}7}$ &$3\times10^{\mbox{-}7}$ \\
BN\_111 &-1.28 &0.14 &$7\times10^{\mbox{-}8}$ &-$2\times10^{\mbox{-}7}$ \\
BN\_113 &-1.75 &-0.11 &$2\times10^{\mbox{-}7}$ &0 \\
BN\_2 &-7.52 &-0.02 &0.10 &$4\times10^{\mbox{-}7}$ \\
BN\_22 &-304.14 &0.66 &$6\times10^{\mbox{-}8}$ &0 \\
BN\_23 &-304.14 &0.66 &$6\times10^{\mbox{-}8}$ &0 \\
BN\_24 &-297.7 &\textbf{4.07} &$2\times10^{\mbox{-}7}$ &-$7\times10^{\mbox{-}7}$ \\
BN\_25 &-297.7 &\textbf{4.07} &$2\times10^{\mbox{-}7}$ &-$7\times10^{\mbox{-}7}$ \\
BN\_30 &-10.99 &-0.21 &3.05 &-$4\times10^{\mbox{-}7}$ \\
BN\_31 &-10.99 &-0.21 &4.59 &-$4\times10^{\mbox{-}7}$ \\
BN\_32 &-11.55 &-0.20 &4.42 &-$2\times10^{\mbox{-}7}$ \\
BN\_33 &-11.55 &-0.20 &4.88 &-$2\times10^{\mbox{-}7}$ \\
BN\_34 &-14.39 &0.55 &3.26 &$1\times10^{\mbox{-}7}$ \\
BN\_35 &-14.39 &0.51 &3.92 &$1\times10^{\mbox{-}7}$ \\
BN\_36 &-9.26 &-1.11 &2.83 &$2\times10^{\mbox{-}7}$ \\
BN\_37 &-9.26 &-1.11 &3.51 &$2\times10^{\mbox{-}7}$ \\
BN\_38 &-10.29 &-1.41 &3.95 &0 \\
BN\_39 &-10.29 &-1.42 &4.49 &0 \\
BN\_40 &-13.21 &-1.73 &2.82 &$7\times10^{\mbox{-}8}$ \\
BN\_41 &-13.21 &-1.73 &1.83 &$7\times10^{\mbox{-}8}$ \\
BN\_42 &-2.37 &-0.16 &0.20 &-$5\times10^{\mbox{-}7}$ \\
BN\_43 &-2.31 &-0.51 &0.47 &-$4\times10^{\mbox{-}5}$ \\
BN\_44 &-3.69 &-0.05 &0.18 &-$8\times10^{\mbox{-}7}$ \\
BN\_45 &-1.89 &-0.56 &0.07 &$1\times10^{\mbox{-}6}$ \\
BN\_46 &-2.72 &$3\times10^{\mbox{-}5}$ &0.40 &$7\times10^{\mbox{-}7}$ \\
BN\_47 &-2.08 &-0.15 &- &-$5\times10^{\mbox{-}8}$ \\
BN\_48 &-2.08 &-0.15 &- &-$5\times10^{\mbox{-}8}$ \\
BN\_49 &-1.72 &-0.09 &- &$7\times10^{\mbox{-}7}$ \\
BN\_50 &-1.72 &-0.09 &- &$7\times10^{\mbox{-}7}$ \\
BN\_51 &-1.43 &-0.08 &- &$2\times10^{\mbox{-}7}$ \\
BN\_52 &-1.43 &-0.08 &- &$2\times10^{\mbox{-}7}$ \\
BN\_53 &-1.13 &0.007 &- &$2\times10^{\mbox{-}7}$ \\
BN\_54 &-1.13 &0.007 &- &$7\times10^{\mbox{-}6}$ \\
BN\_55 &-1.74 &0.02 &- &$7\times10^{\mbox{-}7}$ \\
BN\_56 &-1.74 &0.02 &- &$7\times10^{\mbox{-}7}$ \\
BN\_57 &-1.93 &0.005 &- &$2\times10^{\mbox{-}6}$ \\
BN\_58 &-1.93 &0.005 &- &$2\times10^{\mbox{-}6}$ \\
BN\_59 &-2.47 &-0.28 &- &$1\times10^{\mbox{-}7}$ \\
BN\_60 &-2.47 &-0.28 &- &$1\times10^{\mbox{-}7}$ \\
BN\_61 &-1.71 &0.03 &- &$1\times10^{\mbox{-}6}$ \\
BN\_62 &-1.71 &0.03 &- &$1\times10^{\mbox{-}6}$ \\
BN\_63 &-0.73 &0.02 &- &-$4\times10^{\mbox{-}5}$ \\
BN\_64 &-0.73 &0.02 &- &-$1\times10^{\mbox{-}5}$ \\
BN\_65 &-1.07 &-0.30 &- &$5\times10^{\mbox{-}8}$ \\
BN\_66 &-1.07 &-0.30 &- &$5\times10^{\mbox{-}8}$ \\
BN\_67 &-0.49 &-0.01 &- &-$5\times10^{\mbox{-}5}$ \\
BN\_68 &-0.49 &-0.01 &- &-$1\times10^{\mbox{-}5}$ \\
BN\_8 &-2.39 &0.003 &0.15 &$4\times10^{\mbox{-}6}$ \\
\midrule
\rowcolor{gray!30}{\it \bf Mean $\mathbf{|\Delta_{Alg}|}$} & & {\it \bf 0.48} &{\it \bf 1.62} &\textbf{\it $\mathbf{4 \times 10^{\mbox{-}6}}$} \\
\bottomrule
\end{tabular}%
}
\end{table}

%\begin{table}[!htp]\centering
%	\caption{Probability of evidence obtained using different inference algorithms. $PR_{ACE}$ is logarithm of the exact probability obtained using Ace and $\Delta_{algo}$ is the error in the log probabilities ($PR_{algo}-PR_{ACE}$) obtained using various approximate inference techniques.}\label{tab:pr.bnuai.ace}
%	\scriptsize
%	\begin{tabular}{cccccc}\toprule
%		\textbf{Benchmark} &\textbf{$PR_{ACE}$} &\textbf{$\Delta_{FBP}$} &\textbf{$\Delta_{WMB}$} &\textbf{$\Delta_{Proposed}$} \\\midrule
%\begin{tabular}{cccccc}\toprule
%\textbf{Benchmark} &\textbf{$PR_{ACE}$} &\textbf{$\Delta_{FBP}$} &\textbf{$\Delta_{WMB}$} &\textbf{$\Delta_{Proposed}$} \\\midrule
%BN\_105 &-0.83 &0.12 &0.00 &0.00 \\
%BN\_107 &-1.15 &-0.07 &0.22 &0.00 \\
%BN\_109 &-1.89 &-0.20 &0.00 &0.00 \\
%BN\_111 &-1.28 &0.14 &0.00 &0.00 \\
%BN\_113 &-1.75 &-0.11 &0.00 &0.00 \\
%BN\_2 &-7.52 &-0.02 &0.10 &0.00 \\
%BN\_22 &-304.14 &0.66 &0.00 &0.00 \\
%BN\_23 &-304.14 &0.66 &0.00 &0.00 \\
%BN\_24 &-297.70 &4.07 &0.00 &0.00 \\
%BN\_25 &-297.70 &4.07 &0.00 &0.00 \\
%BN\_30 &-10.99 &-0.21 &3.05 &0.00 \\
%BN\_31 &-10.99 &-0.21 &4.59 &0.00 \\
%BN\_32 &-11.55 &-0.20 &4.42 &0.00 \\
%BN\_33 &-11.55 &-0.20 &4.88 &0.00 \\
%BN\_34 &-14.39 &0.55 &3.26 &0.00 \\
%BN\_35 &-14.39 &0.51 &3.92 &0.00 \\
%BN\_36 &-9.26 &-1.11 &2.83 &0.00 \\
%BN\_37 &-9.26 &-1.11 &3.51 &0.00 \\
%BN\_38 &-10.29 &-1.41 &3.95 &0.00 \\
%BN\_39 &-10.29 &-1.42 &4.49 &0.00 \\
%BN\_40 &-13.21 &-1.73 &2.82 &0.00 \\
%BN\_41 &-13.21 &-1.73 &1.83 &0.00 \\
%BN\_42 &-2.37 &-0.16 &0.20 &0.00 \\
%BN\_43 &-2.31 &-0.51 &0.47 &0.00 \\
%BN\_44 &-3.69 &-0.05 &0.18 &0.00 \\
%BN\_45 &-1.89 &-0.56 &0.07 &0.00 \\
%BN\_46 &-2.72 &0.00 &0.40 &0.00 \\
%BN\_47 &-2.08 &-0.15 &- &0.00 \\
%BN\_48 &-2.08 &-0.15 &- &0.00 \\
%BN\_49 &-1.72 &-0.09 &- &0.00 \\
%BN\_50 &-1.72 &-0.09 &- &0.00 \\
%BN\_51 &-1.43 &-0.08 &- &0.00 \\
%BN\_52 &-1.43 &-0.08 &- &0.00 \\
%BN\_53 &-1.13 &0.00 &- &0.00 \\
%BN\_54 &-1.13 &0.00 &- &0.00 \\
%BN\_55 &-1.74 &0.02 &- &0.00 \\
%BN\_56 &-1.74 &0.02 &- &0.00 \\
%BN\_57 &-1.93 &0.00 &- &0.00 \\
%BN\_58 &-1.93 &0.00 &- &0.00 \\
%BN\_59 &-2.47 &-0.28 &- &0.00 \\
%BN\_8 &-2.39 &0.00 &0.15 &0.00 \\ \hline
%\rowcolor{gray!30}\textbf{\it Mean Error} & &\textbf{\it -0.03} &\textbf{\it 1.62} &\textbf{\it 0.00} \\
%\bottomrule
%\end{tabular}
%\end{table}


==> tables/priormar.bnuai.ace.abs.tex <==
% !TeX spellcheck = en_US

\begin{table}[!htp]\centering
    \caption{Comparison of the maximum error, RMSE and the runtime required (in seconds) to obtain prior marginals for BN\_UAI. Entries are marked with `-' where inference fails. For consistency in precision across algorithms, the error is reported as zero if accurate to three decimal places.}
	\label{tab:priormar.bnuai.ace.abs}
	\scriptsize
	\setlength\tabcolsep{3pt}
	\resizebox{0.45\paperheight}{!}{%
	%\begin{tabular}{l|rrrrr|rrrrr|rrrrrrr}\toprule
	\begin{tabular}{|l|ccc>{\columncolor{gray!30}}c|ccc>{\columncolor{gray!30}}c|cccc>{\columncolor{gray!30}}c|}\toprule
        \multirow{2}{*}{\textbf{Benchmark}} &\multicolumn{4}{c|}{\textbf{max Error}} &\multicolumn{4}{c|}{\textbf{RMSE}} &\multicolumn{5}{c|}{\textbf{Runtime (s)}} \\\cmidrule{2-14}
		&\textbf{FBP} &\textbf{WMB} &\textbf{IJGP} &\textbf{IBIA} &\textbf{FBP} &\textbf{WMB} &\textbf{IJGP} &\textbf{IBIA} &\textbf{ACE} &\textbf{FBP} &\textbf{WMB} &\textbf{IJGP} &\textbf{IBIA} \\\midrule
    BN\_105 &0.24 &0.197 &0.357 &0 &0.074 &0.057 &0.104 &0 &7 &2126 &344 &269 &11 \\
    BN\_107 &0.082 &0.209 &0.683 &0 &0.024 &0.084 &0.239 &0 &6 &1453 &294 &270 &9 \\
    BN\_109 &0.096 &0.122 &0.697 &0 &0.026 &0.028 &0.338 &0 &5 &1189 &328 &246 &8 \\
    BN\_111 &0.279 &0.284 &0.61 &0 &0.074 &0.085 &0.269 &0 &5 &1149 &307 &250 &7 \\
    BN\_113 &0.097 &0.095 &0.703 &0 &0.022 &0.027 &0.234 &0 &6 &1359 &294 &238 &8 \\
    BN\_115 &0.002 &0.038 &0.55 &0.001 &0 &0.008 &0.312 &0 &429 &457 &370 &222 &6 \\
    BN\_117 &0.002 &0.052 &0.525 &0.001 &0 &0.01 &0.327 &0 &552 &920 &346 &234 &9 \\
    BN\_119 &0.003 &0.029 &0.627 &0.001 &0.001 &0.005 &0.32 &0 &348 &395 &327 &211 &5 \\
    BN\_121 &0.001 &0.026 &0.501 &0.001 &0 &0.005 &0.324 &0 &418 &515 &341 &241 &6 \\
    BN\_123 &0.001 &0.039 &0.655 &0.001 &0 &0.007 &0.308 &0 &583 &816 &340 &244 &7 \\
    BN\_125 &0.001 &0.036 &0.534 &0.001 &0 &0.009 &0.306 &0 &483 &346 &393 &244 &5 \\
    BN\_20 &0.15 &0 &0 &0 &0.014 &0 &0 &0 &4515 &3 &166 &112 &10 \\
    BN\_21 &0.15 &0 &0 &0.06 &0.014 &0 &0 &0.001 &5944 &4 &168 &109 &11 \\
    BN\_22 &0.271 &0 &0 &0 &0.01 &0 &0 &0 &4 &3 &21 &12 &5 \\
    BN\_23 &0.271 &0 &0 &0 &0.01 &0 &0 &0 &7 &4 &59 &11 &5 \\
    BN\_24 &0.702 &0 &0 &0 &0.109 &0 &0 &0 &4 &8 &9 &8 &4 \\
    BN\_25 &0.702 &0 &0 &0 &0.109 &0 &0 &0 &6 &8 &10 &8 &3 \\
    BN\_30 &0.606 &0.58 &- &0 &0.138 &0.156 &- &0 &93 &0.1 &770 &- &4 \\
    BN\_31 &0.606 &0.64 &0.74 &0 &0.138 &0.138 &0.265 &0 &65 &0.1 &871 &552 &4 \\
    BN\_32 &0.558 &0.615 &- &0 &0.152 &0.16 &- &0 &143 &0.1 &940 &- &5 \\
    BN\_33 &0.558 &0.657 &0.997 &0 &0.152 &0.156 &0.301 &0 &96 &0.1 &992 &742 &5 \\
    BN\_34 &0.558 &0.556 &- &0 &0.152 &0.162 &- &0 &900 &0.1 &955 &- &5 \\
    BN\_35 &0.558 &0.788 &- &0 &0.152 &0.168 &- &0 &276 &0.1 &924 &- &5 \\
    BN\_36 &0.558 &0.622 &- &0 &0.152 &0.186 &- &0 &845 &0.1 &1013 &- &5 \\
    BN\_37 &0.558 &0.645 &- &0.002 &0.152 &0.183 &- &0 &1316 &0.1 &1086 &- &5 \\
    BN\_38 &0.558 &0.628 &- &0 &0.152 &0.172 &- &0 &798 &0.1 &964 &- &5 \\
    BN\_39 &0.558 &0.648 &0.807 &0.001 &0.152 &0.173 &0.262 &0 &2820 &0.1 &1085 &740 &5 \\
    BN\_40 &0.558 &0.599 &- &0.001 &0.152 &0.161 &- &0 &66 &0.1 &1113 &- &5 \\
    BN\_41 &0.558 &0.599 &- &0.001 &0.152 &0.173 &- &0 &202 &0.1 &1000 &- &5 \\
    BN\_42 &0.072 &0.122 &0.75 &0.03 &0.026 &0.027 &0.111 &0.001 &508 &0.01 &91 &74 &1 \\
    BN\_43 &0.072 &0.113 &0.75 &0.004 &0.026 &0.032 &0.115 &0 &723 &0.01 &95 &74 &2 \\
    BN\_44 &0.072 &0.104 &0.316 &0.004 &0.026 &0.024 &0.056 &0 &677 &0.01 &103 &69 &1 \\
    BN\_45 &0.072 &0.126 &0.75 &0.004 &0.026 &0.039 &0.137 &0 &416 &0.01 &81 &75 &1 \\
    BN\_46 &0.022 &0.239 &0.5 &0 &0.003 &0.036 &0.207 &0 &39 &0.01 &109 &91 &1 \\
    BN\_47 &0.125 &0.271 &0.969 &0.028 &0.017 &0.084 &0.353 &0.003 &1 &0.1 &675 &557 &4 \\
    BN\_48 &0.125 &0.286 &0.938 &0.03 &0.017 &0.088 &0.307 &0.002 &1 &0.1 &771 &531 &3 \\
    BN\_49 &0.125 &0.274 &0.969 &0.046 &0.017 &0.081 &0.349 &0.003 &1 &0.1 &650 &526 &3 \\
    BN\_50 &0.125 &0.298 &0.969 &0.022 &0.017 &0.098 &0.337 &0.002 &1 &0.1 &677 &553 &3 \\
    BN\_51 &0.125 &0.299 &0.969 &0.034 &0.017 &0.096 &0.334 &0.003 &1 &0.1 &820 &516 &3 \\
    BN\_52 &0.125 &0.256 &0.953 &0.019 &0.017 &0.087 &0.323 &0.002 &1 &0.1 &738 &602 &3 \\
    BN\_53 &0.103 &0.452 &0.992 &0.022 &0.018 &0.147 &0.299 &0.002 &1 &0.01 &495 &413 &3 \\
    BN\_54 &0.103 &0.445 &0.992 &0.044 &0.018 &0.135 &0.305 &0.005 &1 &0.01 &436 &307 &3 \\
    BN\_55 &0.103 &0.477 &0.992 &0.026 &0.018 &0.135 &0.327 &0.002 &1 &0.02 &439 &414 &3 \\
    BN\_56 &0.103 &0.453 &- &0.044 &0.018 &0.13 &- &0.005 &1 &0.03 &572 &- &4 \\
    BN\_57 &0.103 &0.42 &0.992 &0.044 &0.018 &0.123 &0.302 &0.003 &1 &0.01 &508 &395 &3 \\
    BN\_58 &0.103 &0.416 &0.938 &0.044 &0.018 &0.128 &0.322 &0.003 &2 &0.01 &484 &403 &3 \\
    BN\_59 &0.125 &0.449 &0.938 &0.012 &0.018 &0.134 &0.298 &0.001 &1 &0.02 &568 &396 &5 \\
    BN\_60 &0.125 &0.457 &- &0.07 &0.018 &0.143 &- &0.006 &2 &0.02 &550 &- &3 \\
    BN\_61 &0.141 &0.337 &0.891 &0.036 &0.017 &0.082 &0.324 &0.003 &0 &0.1 &707 &558 &4 \\
    BN\_62 &0.141 &0.287 &0.891 &0.056 &0.017 &0.085 &0.329 &0.004 &1 &0.1 &709 &540 &3 \\
    BN\_63 &0.125 &0.442 &0.938 &0.072 &0.018 &0.137 &0.319 &0.003 &2 &0.02 &486 &465 &4 \\
    BN\_64 &0.125 &0.504 &0.992 &0.011 &0.018 &0.146 &0.337 &0.001 &2 &0.02 &553 &404 &3 \\
    BN\_65 &0.133 &0.763 &0.75 &0.07 &0.013 &0.248 &0.196 &0.004 &1 &0.01 &401 &278 &4 \\
    BN\_66 &0.133 &0.765 &0.875 &0.113 &0.013 &0.243 &0.216 &0.007 &1 &0.01 &385 &296 &5 \\
    BN\_67 &0.133 &0.771 &0.875 &0.088 &0.013 &0.246 &0.208 &0.006 &1 &0.01 &382 &336 &4 \\
    BN\_68 &0.133 &0.787 &0.75 &0.096 &0.013 &0.256 &0.202 &0.006 &3 &0.01 &383 &343 &4 \\
    BN\_86 &0 &0 &0.487 &0 &0 &0 &0.03 &0 &34 &77 &227 &133 &2 \\
    BN\_87 &0 &0 &0.487 &0 &0 &0 &0.03 &0 &51 &63 &229 &126 &2 \\
    BN\_88 &0 &0 &0.487 &0 &0 &0 &0.03 &0 &34 &52 &213 &131 &2 \\
    BN\_89 &0 &0 &0.487 &0 &0 &0 &0.03 &0 &53 &114 &242 &114 &3 \\
    BN\_90 &0 &0 &0.5 &0 &0 &0 &0.038 &0 &36 &77 &214 &124 &2 \\
    BN\_91 &0 &0 &0.357 &0 &0 &0 &0.018 &0 &49 &128 &202 &123 &2 \\
    BN\_92 &0 &0.005 &0.357 &0 &0 &0 &0.018 &0 &34 &70 &186 &123 &3 \\
    BN\_93 &0 &0 &0.487 &0 &0 &0 &0.03 &0 &52 &76 &304 &149 &3 \\ \midrule
    \rowcolor{gray!30}{\bf Mean} &{\bf 0.201} &{\bf 0.302} &{\bf 0.647} &{\bf 0.018} &{\bf 0.043}  &{\bf 0.086} &{\bf 0.203} &{\bf 0.001} &\multicolumn{5}{c|}{} \\
    \bottomrule
	\end{tabular}%
	}
\end{table}


==> tikz/approxCTF.tex <==

\begin{figure}[htb]
\centering
    \captionsetup[subfigure]{position=b}
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \input{tikz/approx-step1}
        \caption{Step1: Selecting minimal subgraph of CTF that connects interface variables (marked in red).}
        \label{fig:approxStep1}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \input{tikz/approx-step2}
        \caption{Step2a: Exact marginalization of non-interface variables present in a single clique.}
        \label{fig:approxStep2a}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \input{tikz/approx-step2b}
        \caption{Step2b: Exact marginalize NIVs present in multiple cliques such that $mcs\leq mcs_{im}=3$.}
        \label{fig:approxStep2b}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \input{tikz/approx-step3}
        \caption{Step3: Trim cliques with size $>mcs_{im}$ (highlighted in red) using local marginalization. The cliques in which the variable is retained are outlined.}
        \label{fig:approxStep3}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \input{tikz/approx-step4}
        \caption{Step4: Find interface map between the partition $CTF_1$ and the approximate $CTF_a$.}
        \label{fig:approxStep4}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \input{tikz/approx-step5}
        \caption{Step5: Re-assign clique factors ($\psi$) using clique $fhm$ as the root node.}
        \label{fig:approxStep5}
    \end{subfigure}%
    \caption{Steps involved in approximating partition $CTF_1$ of the example BN to obtain $CTF_a$ with maximum clique size $mcs_{im}=3$ using Algorithm~\ref{alg:ApproximateCTF}.}
    \label{fig:approxCTF}
\end{figure}


==> tikz/buildCase1.tex <==
\begin{figure}[t]
	\small
	\centering
	\captionsetup[subfigure]{position=b}
	\begin{subfigure}[t]{0.3\textwidth}
		\centering
		\begin{tikzpicture}[thick,scale=0.8, every node/.style={transform shape}]
            \foreach \pos/\name/\label in {(0,0)/$C:~abe$/abe, (2,0)/$C_1:~c$/c, (4,0)/$C_2:~d$/d}
            \node [vertexr] (\label) at \pos {\name};
            \foreach \pos/\name/\label in {(0,-1.5)/$C_v:~abf$/abf}
            \node [selected vertext] (\label) at \pos {\name};
            \path[edge2] (abe) -- node [right, midway] {\color{gray} $ab$}(abf);
        \end{tikzpicture}
		%\begin{tikzpicture}[thick,scale=0.8, every node/.style={transform shape}]
        %    \foreach \pos/\name/\label in {((4,0)/$C_2:~d$/d, (2,0)/$C_1:~c$/c}
        %    \node [vertexr] (\label) at \pos {\name};
        %    \foreach \pos/\name/\label in {(0,0)/$C:~{\color{blue}\boldsymbol{ab}}e$/abe}
        %    \node [selected vertex] (\label) at \pos {\name};
        %   % \path[edge2] (abe) -- node [right, midway] {\color{gray} $ab$}(abf);
        %    \node (d1) at (0,-1.75) {};
		%\end{tikzpicture}
        %\caption{Existing CT. Impacted subgraph $SG_{min}$ is highlighted in red.}
	\end{subfigure}%
    \hfill
	\begin{subfigure}[t]{0.3\textwidth}
		\centering
		\begin{tikzpicture}[thick,scale=0.8, every node/.style={transform shape}]
		\end{tikzpicture}
        %    \foreach \pos/\name/\label in {(0,0)/$C:~abe$/abe, (2,0)/$C_1:~c$/c, (4,0)/$C_2:~d$/d}
        %    \node [vertexr] (\label) at \pos {\name};
        %    \foreach \pos/\name/\label in {(0,-1.5)/$C_v:~abf$/abf}
        %    \node [selected vertext] (\label) at \pos {\name};
        %    \path[edge2] (abe) -- node [right, midway] {\color{gray} $ab$}(abf);
		%\end{tikzpicture}
		%\caption{Modified CT}
	\end{subfigure}
    \caption{\textit{\underline{Case 1}}: Addition of a new variable ($f$) with both parents ($a,~b$) present in the same clique in the existing CT.}
	\label{fig:mCF1}
\end{figure}

